Video Description using Bidirectional Recurrent Neural Networks

Although traditionally used in the machine translation field, the encoder-decoder framework has been recently applied for the generation of video and image descriptions. The combination of Convolutional and Recurrent Neural Networks in these models has proven to outperform the previous state of the art, obtaining more accurate video descriptions. In this work we propose pushing further this model by introducing two contributions into the encoding stage. First, producing richer image representations by combining object and location information from Convolutional Neural Networks and second, introducing Bidirectional Recurrent Neural Networks for capturing both forward and backward temporal relationships in the input frames.

==> IEEE_files/1_introduction.tex <==
\section{Introduction}
% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.
\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
for IEEE journal papers produced under \LaTeX\ using
IEEEtran.cls version 1.8b and later.
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)
I wish you the best of success.

\subsection{Subsection Heading Here}
Subsection text here.

% needed in second column of first page if using \IEEEpubid
%\IEEEpubidadjcol

\subsubsection{Subsubsection Heading Here}
Subsubsection text here.

==> IEEE_files/2_related_work.tex <==
\section{Related Work}

Although the problem of video captioning has just recently appeared thanks to the new learning capabilities offered by Deep Learning, the general pipeline used in these works resembles the traditional encoder-decoder methodology used in machine translation. The main difference in this case is that in the encoder step, instead of generating a compact representation of the source language sentence, we generate a representation of the images belonging to the source video.

In this section we will review the most important related works in the state of the art that work on machine translation and image representation separately, and then the works devoted to image captioning and video captioning.



\subsection{Machine Translation and Recurrent Neural Networks}

Despite that the idea of applying neural networks in the Machine Translation (MT) field is not new~\cite{Castano97}, the application of connectionist, continuous models has obtained much attention from the researchers in the last few years. The seminal work of this new approach to the natural language processing (NLP) was a neural language model~\cite{Bengio03}, where words were projected from their original discrete representation to a continuous, real-valued one. Word probabilities were estimated over the continuous space. From here, many others followed this approach, applying neural networks to deploy language models~\cite{Mikolov10, Sundermeyer12} and translation models~\cite{Schwenk12, Devlin14}, which were included in the classic phrase-based pipeline~\cite{Koehn03}.

Furthermore, a new approach to MT was recently developed, the so-called Neural Machine Translation (NMT), where the translation process is carried out by a single, large neural network~\cite{Sutskever14, Cho14}. NMT systems rely on the encoder-decoder framework: An encoder recurrent neural network (RNN) produces a continuous representation of an input sentence in the source language. The decoder RNN takes this representation and generates the corresponding target language sentence. Later works included an attention mechanism to the model~\cite{Bahdanau15}, which allowed the decoder to selectively focus on parts of the input sequence and increased the performance on long input sentences. % TODO: UNK_replace

\textcolor{blue}{Marc: maybe we should also introduce the LSTM units?}
\textcolor{blue}{Paco: yes only a brief comment but the formal introduction in Section III}
\textcolor{blue}{Paco: maybe a short reference at the begining of the this subsection to the state-of-the art in MT would be welcome}

\subsection{Image and Video Representation}

The recent re-introduction of Deep Learning in the Computer Vision field through the use of Convolutional Neural Networks (CNN) \cite{krizhevsky2012imagenet}, has allowed to obtain new and richer image representations compared to the traditional hand-crafted ones. This burst has been possible thanks to the appearance of huge image databases and the possibility of large-scale training with GPUs.

These networks have demonstrated to be a powerful tool to extract feature representations for several kinds of recognition and localization problems like objects \cite{krizhevsky2012imagenet, ren2015faster}, scenes \cite{zhou2014learning},  faces \cite{lawrence1997face}, text \cite{wang2012end,goodfellow2013multi}, etc.

Additionally, and even more recently, CNNs has also been applied not only for single images but on videos for either category classification \cite{karpathy2014large} or activity recognition \cite{tran2014learning}.

Thanks to the CNNs ability to serve as knowledge transfer mechanisms \cite{zhou2014object}, they have been usually used as feature extractors simply by removing the classification layer of the chosen network (which will be specifically designed for a particular problem). By doing this, we can use the output of the last fully connected \cite{dimiccoli2015sr} or convolutional layers \cite{zhou2014object} as a feature vector applicable to other related but not strictly equal problems. In other cases also several intermediate layers have been used for building a more complete representation \cite{Salvador_2015_CVPR_Workshops}.



\subsection{Image Captioning}

The majority of the works devoted to generate textual descriptions from single images follow a clear model architecture. In the encoding step they apply a CNN for describing the input image, and in the decoding step an LSTM is in charge of receiving the image information at the first time step and generate an ordered sequence of words at each time step producing a final sentence description (\textcolor{blue}{Marc: show figure with a simple example?} \textcolor{blue}{Paco: I think so}). We will name as CNN-LSTM this basic architecture on the rest of the paper.

Although maintaining the described architectural core, this methodology, which was popularized by Vinyals et al. \cite{vinyals2015show}, has experienced several modifications and proposals by different groups. In \cite{klein2014fisher}, instead of using a one-hot vector representation of the previously generated word as an input to the LSTM at each time step, the authors propose using the word2vec representation \cite{mikolov2013distributed} of the words followed by learning a Fisher Vector \cite{perronnin2007fisher} representation on them. Additionally, they map both the images and words into a common space by using the CCA algorithm. In \cite{karpathy2015deep} the authors use the CNN-LSTM methodology but in this case not only for generating captions for complete images, but also short snippets for specific regions in the image. Another alternative model was proposed in \cite{xu2015show}, where an Attention mechanism is used. The attention capabilities of the model are based on the spatial information extracted from the convolutional layers of the CNN. This mechanism allows the model to iteratively change its point of focus on the image at each time step and, consequently, decide which is the most relevant region for generating the next word.

\textcolor{blue}{Paco: references to other works with other approaches (no CNN)?}

\subsection{Video Captioning}

Some works have also been presented for the similar problem of video captioning. Although, the seminal papers devoted to this topic tried a different approach compared to the usual architecture described for image captioning. Both in \cite{krishnamoorthy2013generating} and \cite{rohrbach2013translating} the authors applied methodologies more similar to the classical machine translation problems. Detecting a set of relevant concepts in the encoding step, being either $<$Subject, Verb, Object$>$ triplets in the former or sets of semantic concepts like $<$Activity, Tool, Object, Source, Target$>$ in the latter. And treat it as a translation problem in the decoding step by generating an associated sentence.

Other more recent works in the state of the art have also followed the same CNN-LSTM model architecture as a basis due to its high performance. Venugopalan et al. in \cite{venugopalan2014translating} propose extracting CNN features from each image in the video and applying a mean on the result for representing the whole video. Additionally, in the decoder, they use a two-layered LSTM structure whose input in each time step is both the previously generated word and the encoded video. More recently, the same authors presented in \cite{venugopalan2015sequence} a different approach. The main contribution is that instead of using a single CNN for representing the video frames, they combine the features of a CNN trained on raw images for object classification and a CNN trained on optical flow for activity recognition. The work that has obtained better results so far is the one from Yao et al. \cite{yao2015describing}. They also follow the CNN-LSTM architecture but in this case adding two contributions. The first one, following the ideas in \cite{venugopalan2015sequence}, is to add a CNN for activity recognition using a 3D-CNN, which has the ability to capture temporal relationships between close frames. The second one, similar to \cite{xu2015show}, is to add an attention mechanism that learns where does it have to focus at each time step. Even though, in this case, they propose using a temporal mechanism, which focuses in different frames of the video depending on the last generated words.




\subsection{Our Contributions}

Text



==> IEEE_files/3_methodology.tex <==
\section{Methodology}
Text


==> IEEE_files/4_results.tex <==
\section{Results}
Text


==> IEEE_files/5_discussion.tex <==
\section{Discussion}
Text



==> IEEE_files/6_conclusions.tex <==
\section{Conclusions}
Text
